Improved Communication-Privacy Trade-offs in $L_2$ Mean Estimation under Streaming Differential Privacy

We study $L_2$ mean estimation under central differential privacy and communication constraints, and address two key challenges: firstly, existing mean estimation schemes that simultaneously handle both constraints are usually optimized for $L_\infty$ geometry and rely on random rotation or Kashin's representation to adapt to $L_2$ geometry, resulting in suboptimal leading constants in mean square errors (MSEs); secondly, schemes achieving order-optimal communication-privacy trade-offs do not extend seamlessly to streaming differential privacy (DP) settings (e.g., tree aggregation or matrix factorization), rendering them incompatible with DP-FTRL type optimizers. In this work, we tackle these issues by introducing a novel privacy accounting method for the sparsified Gaussian mechanism that incorporates the randomness inherent in sparsification into the DP noise. Unlike previous approaches, our accounting algorithm directly operates in $L_2$ geometry, yielding MSEs that fast converge to those of the uncompressed Gaussian mechanism. Additionally, we extend the sparsification scheme to the matrix factorization framework under streaming DP and provide a precise accountant tailored for DP-FTRL type optimizers. Empirically, our method demonstrates at least a 100x improvement of compression for DP-SGD across various FL tasks.

==> figures/plot_style.tex <==
emnist_cdp_rootdir = '/cns/lu-d/home/weiningc/dp_train/66829641-dp_compression_sonwp_large_n'

val_acc_name = 'evaluation/eval/accuracy_without_out_of_vocab_or_end_of_sentence'
train_acc_name = 'train/accuracy_without_out_of_vocab_or_end_of_sentence'
val_loss_name = 'evaluation/eval/loss'
train_loss_name = 'train/loss'

val_window_size = 5

clip_norm = 0.3
epsilon_list = [3.0]
sparsification_rate_list = [1.0, 0.01, 0.005, 0.001]
server_learning_rate_list = [1.0]


from IPython.display import clear_output
import copy
import glob

import matplotlib
import matplotlib.pyplot as plt
from matplotlib import rcParams
import matplotlib.gridspec as gridspec
matplotlib.use('Agg')
%matplotlib inline

import numpy as np
import os


import warnings
warnings.filterwarnings('ignore')

color_list = ['tab:blue',
             'tab:orange',
             'tab:green',
             'tab:red',]

fig = plt.figure(figsize=(18, 8), dpi=144)
gs = gridspec.GridSpec(2, 4)
ax1 = fig.add_subplot(gs[0, 0])
ax2 = fig.add_subplot(gs[0, 1])

params={'legend.fontsize': 10, 'legend.handlelength':1}
sns.set_context('paper', font_scale=2)
sns.set_style('whitegrid')
fig=plt.figure()

######################### First figure #########################
for eps in epsilon_list:

  for server_learning_rate in server_learning_rate_list:
    for sparsification_rate in sparsification_rate_list:
      cdp_dirs = glob_dirs(emnist_cdp_rootdir, [f'epsilon={eps}', f'sparsification_rate={sparsification_rate}', f'l2_norm_clip={clip_norm}', f'server_learning_rate={server_learning_rate}'])
      print('DIRS'); pprint.pprint(cdp_dirs);
      cdp_val_accs = parse_metric(cdp_dirs[0], val_acc_name, val_window_size, last=False)
      cdp_val_losses = parse_metric(cdp_dirs[0], val_loss_name, val_window_size, last=False)
      round_list = [val_window_size*i for i in range(len(cdp_val_accs))]
      label = 'no compression'
      linestyle = '--'
      if sparsification_rate!= 1.0:
        compression_rate = int(1/sparsification_rate)
        label = str(compression_rate)+'x'
        linestyle = '-'
      ax1.plot(round_list[::5], cdp_val_accs[::5], linewidth=2, label=label, linestyle = linestyle)

    ax1.set_xlabel('Rounds', fontsize=18)
    ax1.set_ylabel('Accuracy', fontsize=18)
    ax1.tick_params(axis='both', which='major', labelsize=12)
    ax1.legend(prop={'size': 10}, loc='lower right')

    ax1.set_title(f'Stackoverflow Word', fontsize=18)
    ax1.grid()
    ax1.grid('on')

######################### Second figure #########################
emnist_cdp_rootdir = '/cns/ue-d/home/weiningc/dp_train/67179651-dp_compression_emnist_eps_sweep'
val_acc_name = 'evaluation/eval/sparse_categorical_accuracy'
train_acc_name = 'train/sparse_categorical_accuracy'
val_loss_name = 'evaluation/eval/loss'
train_loss_name = 'train/loss'

val_window_size = 20

clip_norm = 0.03
epsilon_list = [1.0, 3.0, 5.0, 7.0, 9.0]
sparsification_rate_list = [1.0,  1/800, 1/1600, 1/3200]

acc_dic = {}
loss_dic = {}

for eps in epsilon_list:
  for sparsification_rate in sparsification_rate_list:
    cdp_dirs = glob_dirs(emnist_cdp_rootdir, [f'epsilon={eps}',
                                              f'sparsification_rate={sparsification_rate}',
                                              f'l2_norm_clip={clip_norm}',
                                              ])
    print('DIRS'); pprint.pprint(cdp_dirs);
    cdp_val_accs = parse_metric(cdp_dirs[0], val_acc_name, val_window_size, last=True)
    print(cdp_val_accs)
    cdp_val_losses = parse_metric(cdp_dirs[0], val_loss_name, val_window_size, last=True)
    acc_dic[eps, sparsification_rate] = cdp_val_accs
    loss_dic[eps, sparsification_rate] = cdp_val_losses

for sparsification_rate in sparsification_rate_list:
  acc_eps_list = [acc_dic[eps, sparsification_rate] for eps in epsilon_list]
  loss_eps_list = [loss_dic[eps, sparsification_rate] for eps in epsilon_list]
  if sparsification_rate != 1.0:
    linestyle = '-'
    marker = 'o'
  else:
    linestyle = '--'
    marker = 'x'
  if int(1/sparsification_rate) == 1.0:
    label_ = 'no compression'
  else:
    label_ = f'{int(1/sparsification_rate)}x'
  ax2.plot(epsilon_list,
           acc_eps_list,
           linewidth=2,
           label=f'{label_}',
           linestyle=linestyle)



ax2.set_xlabel(r'$\epsilon$', fontsize=18)
ax2.tick_params(axis='both', which='major', labelsize=12)
ax2.legend(prop={'size': 10}, loc='lower right')

ax2.set_title(f'EMNIST-62', fontsize=18)
ax2.grid()
ax2.grid('on')

name = f'combined_emnist_sonwp_eps_{3}_n_1000'
fig.savefig("{}.png" .format(name))
file_id = drive.SaveFile("{}.png" .format(name), open("{}.png" .format(name), 'rb').read(), mime_type='image/png')
print(f'https://drive.google.com/file/d/{file_id}/view')
